Improving the evaluation of samplers on multi-modal targets

Addressing multi-modality constitutes one of the major challenges of sampling. In this reflection paper, we advocate for a more systematic evaluation of samplers towards two sources of difficulty that are mode separation and dimension. For this, we propose a synthetic experimental setting that we illustrate on a selection of samplers, focusing on the challenging criterion of recovery of the mode relative importance. These evaluations are crucial to diagnose the potential of samplers to handle multi-modality and therefore to drive progress in the field.

==> def.tex <==
\newcommand{\prior}{q}

\newcommand{\pushb}[2]{{#1}_{#2^{-1}}}
\newcommand{\wbar}{\overline{W}}
\newcommand{\ybar}{\overline{y}}

\def\mod{\ \mathrm{mod}}

\def \bfX {\mathbf{X}}
\def \bfB {\mathbf{B}}
\def \bfY {\mathbf{Y}}

\def\Qbb {\mathbb{Q}}
\def\Pbb {\mathbb{P}}
\def\Mbb {\mathbb{M}}

\def\argmin{\mathrm{argmin}}
\def\rmM{\mathrm{M}}
\def\rmP{\mathrm{P}}
\def\msf{\mathsf{G}}
\def\msp{\mathsf{P}}
\def\borel{\mathcal{B}}
\def\Pmeasure{\mathscr{P}}
\def\Qker{\mathrm{Q}}
\def\Rker{\mathrm{R}}
\def\Sker{\mathrm{S}}
\def\Pens{\mathscr{P}}
\def\Ltt{\mathtt{L}}
\def\Mtt{\mathtt{M}}
\def\Jac{\mathrm{Jac}}
\def\dom{\mathrm{dom}}
\def\msd{\mathsf{D}}
\def\msw{\mathsf{W}}
\newcommand{\rref}[1]{\textup{\Cref{#1}}}
\def\rmA{\mathrm{A}}
\def\rmB{\mathrm{B}}
\def\msu{\mathsf{U}}
\newcommand{\yazid}[1]{\textcolor{blue}{\textbf{Yazid}: #1}}

\newcommand{\Image}{\text{Im}}
\newcommand{\Ker}{\text{Ker}}
\newcommand{\TM}{\mathrm{T}^\star\msm}
\newcommand{\Th}{\mathrm{S}_{h/2}}
\newcommand{\Rh}{\mathrm{R}_{h}}
\newcommand{\Gh}{\mathrm{G}_{h}}
\newcommand{\ug}{\underline{\mathrm{g}}}
\newcommand{\oGh}{\overline{\mathrm{G}}_{h}}
\newcommand{\uGh}{\underline{\mathrm{G}}_{h}}
\newcommand{\ugh}{\underline{\mathrm{g}}_{h}}
\newcommand{\ughz}{\underline{\mathrm{g}}_{h,z}}
\newcommand{\Fh}{\mathrm{F}_{h}}
\newcommand{\tildeFh}{\tilde{\mathrm{F}}_{h}}
\newcommand{\tildeGh}{\tilde{\mathrm{G}}_{h}}
\newcommand{\In}{\text{I}_n}
\newcommand{\phiRh}{\mathrm{R}_{h}^{\Phi}}
\newcommand{\tildeRh}{\tilde{\mathrm{R}}_{h}}
\newcommand{\msephi}{\bar{\mse}_h^\Phi}
\newcommand{\tildemsephi}{\tilde{\mse}_h^\Phi}
\newcommand{\Tminush}{\mathrm{T}_{-h/2}}
\newcommand*{\myotop}{\perp\mkern-20.7mu\bigcirc}
\newcommand{\TMx}[1]{\mathrm{T}^\star_{#1}\msm}


\def\projM{\operatorname{proj}_{\mathcal{M}(\Qbb^V)}}
\def\projR{\operatorname{proj}_{\mathcal{R}(\Qbb^V)}}

\newcommand{\tcmb}[1]{\textcolor{blue}{#1}}
\newcommand{\tcmo}[1]{\textcolor{orange}{#1}}
\newcommand{\tcmv}[1]{\textcolor{green!60!black}{#1}}
\newcommand{\tcmr}[1]{\textcolor{red}{#1}}
\newcommand{\tcmp}[1]{\textcolor{violet}{#1}}


\def\M{\msm}
\def\vol{\text{vol}}



\def\complementary{\mathrm{c}}
\def\msi{\mathsf{I}}
\def\msa{\mathsf{A}}
\def\msdd{\mathsf{D}}
\def\msk{\mathsf{K}}
\def\msK{\mathsf{K}}
\def\msks{\mathsf{K}^{\star}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\mst{\mathsf{T}}
\def\msl{\mathsf{L}}
\def\msat{\tilde{\mathsf{A}}}
\def\tgamma{\tilde{\gamma}}
\def\msb{\mathsf{B}} 
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{O}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\bmsh{\bar{\msh}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msz{\mathsf{Z}}
\def\msy{\mathsf{Y}}



\def\mca{\mathcal{A}}
\def\mcz{\mathcal{Z}}
\def\bmca{\bar{\mathcal{A}}}
\def\mcd{\mathcal{D}}
\def\mcl{\mathcal{L}}
\def\mcs{\mathcal{S}}
\def\mct{\mathcal{T}}
\def\tmct{\tilde{\mathcal{T}}}
\def\tmcs{\tilde{\mathcal{S}}}
\def\bmcl{\bar{\mathcal{L}}}
\def\bmcs{\bar{\mathcal{S}}}
\def\bmct{\bar{\mathcal{T}}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcbb{\mathcal{B}}  %
\newcommand{\mcb}[1]{\mathcal{B}(#1)}
\def\mcc{\mathcal{C}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\def\tmcr{\tilde{\mathcal{R}}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}


\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}


\def\rmm{\mathrm{m}}
\def\mrm{\mathrm{m}}
\def\rmd{\mathrm{d}}
\def\mrd{\mathrm{d}}
\def\rmf{\mathrm{f}}
\def\mrl{\mathrm{L}}
\def\mrH{\mathrm{H}}
\def\rmH{\mathrm{H}}
\def\rml{\mathrm{L}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrC{\mathrm{C}}
\def\mrCb{\mathrm{C}_{\operatorname{b}}}
\def\rmCb{\mathrm{C}_{\operatorname{b}}}
\def\mrc{\mathrm{c}}
\def\rmc{\mathrm{c}}
\def\rmC{\mathrm{C}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmU{\mathrm{U}}
\def\rmY{\mathrm{Y}}
\def\rmb{\mathrm{b}}

\def\KL{\mathrm{KL}}
\def\ent{\mathrm{H}}

\def\frX{\mathfrak{X}}
\def\frg{\mathfrak{g}}


\newcommand{\absolute}[1]{\left\vert #1 \right\vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\absLigne}[1]{\vert #1 \vert}
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommand{\tvnormEq}[1]{\left \| #1 \right \|_{\mathrm{TV}}}
\newcommand{\Vnorm}[2][1=V]{\| #2 \|_{#1}}
\newcommand{\normpi}[2][2=\mrl^2(\pi)]{\left\Vert  #1 \right\Vert_{#2}}
\newcommand{\normH}[2][2=2]{\left\Vert  #1 \right\Vert}
\newcommand{\normHLigne}[2][2=2]{\Vert  #1 \Vert}
\newcommand{\normHLine}[2][2=2]{\Vert  #1 \Vert}
\newcommand{\normmu}[2][2=2]{\left\Vert  #1 \right\Vert_{#2}}
\newcommand{\normopmu}[2][2=2]{\left\vvvert  #1 \right\vvvert_{#2}}
\newcommand{\normoppi}[2][2=\rml^2(\pi)]{\left\vvvert  #1 \right\vvvert_{#2}}
\newcommand{\normopH}[2][2=2]{\left\vvvert  #1 \right\vvvert}
\newcommand{\normop}[2][2=2]{\left\vvvert  #1 \right\vvvert}
\newcommandx{\psr}[3][3=]{\left\langle#1,#2 \right\rangle_{#3}}
\newcommandx{\normr}[2][2=]{ \left\Vert#1 \right\Vert_{#2}}
\newcommandx{\psrLigne}[3][3=]{\langle#1,#2 \rangle_{#3}}
\newcommandx{\normrLigne}[2][2=]{ \Vert#1 \Vert_{#2}}
\newcommand{\pspi}[2]{\left\langle#1,#2 \right\rangle_2}
\newcommand{\psH}[2]{\left\langle#1,#2 \right\rangle}
\newcommand{\psmu}[2]{\left\langle#1,#2 \right\rangle_2}
\newcommand{\psmuLigne}[2]{\langle#1,#2 \rangle_2}
\newcommand{\normpiLine}[2][2=2]{\Vert  #1 \Vert_{#2}}
\newcommand{\normpiLigne}[2][2=2]{\Vert  #1 \Vert_{#2}}
\newcommand{\normmuLine}[2][2=2]{\Vert  #1 \Vert_{#2}}
\newcommand{\normmuLigne}[2][2=2]{\Vert  #1 \Vert_{#2}}
\newcommand{\normopmuLine}[2][2=2]{\vvvert  #1 \vvvert_{#2}}
\newcommand{\normopmuL}[2][2=2]{\normopmuLine{#1}[#2]}
\newcommand{\normopHLine}[2][2=2]{\vvvert  #1 \vvvert}
\newcommand{\normopLine}[2][2=2]{\vvvert  #1 \vvvert}
\newcommand{\pspiLine}[2]{\langle#1,#2 \rangle_2}
\newcommand{\psmuLine}[2]{\langle#1,#2 \rangle_2}
\newcommand{\VnormEq}[2][1=V]{\left\| #2 \right\|_{#1}}
\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\left\Vert #2 \right\Vert}{\left\Vert #2 \right\Vert^{#1}}}
\newcommand{\normLigne}[1]{\| #1 \|}
\newcommand{\crochet}[1]{\left\langle#1 \right\rangle}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\newcommand{\parentheseLigne}[1]{(#1 )}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\newcommand{\parentheseDeuxLigne}[1]{[ #1 ]}
\newcommand{\defEns}[1]{\left\lbrace #1 \right\rbrace }
\newcommand{\defEnsLigne}[1]{\lbrace #1 \rbrace }
\newcommand{\defEnsPoint}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsPointDeux}[1]{\left. #1 \right  \rbrace }
\newcommand{\defEnsL}[1]{\left\lbrace #1 \right. }
\newcommand{\defEnsR}[1]{\left. #1 \right  \rbrace }

\newcommand{\proba}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\probaLigne}[1]{\mathbb{P}( #1 )}
\newcommand\probaMarkovTilde[2][2=]
{\ifthenelse{\equal{#2}{}}{{\widetilde{\mathbb{P}}_{#1}}}{\widetilde{\mathbb{P}}_{#1}\left[ #2\right]}}
\newcommand{\probaMarkov}[2]{\mathbb{P}_{#1}\left( #2\right)}
\newcommand{\PE}{\mathbb{E}} %
\newcommand{\expe}[2]{\PE_{#1} \left[ #2 \right]}
\newcommand{\expeExpo}[2]{\PE^{#1} \left[ #2 \right]}
\newcommand{\expeLigne}[1]{\PE [ #1 ]}
\newcommand{\expeLine}[1]{\PE [ #1 ]}
\newcommand{\expeMarkov}[2]{\PE_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovLigne}[2]{\PE_{#1} [ #2 ]}
\newcommand{\expeMarkovExpo}[3]{\PE_{#1}^{#2} \left[ #3 \right]}
\newcommand{\probaMarkovTildeDeux}[2]{\widetilde{\mathbb{P}}_{#1} \left[ #2 \right]}
\newcommand{\expeMarkovTilde}[2]{\widetilde{\PE}_{#1} \left[ #2 \right]}


\newcommand{\plusinfty}{+\infty}
\def\ie{\textit{i.e.}}
\def\cadlag{càdlàg}
\def\eqsp{\;}
\def\eqand{\quad \text{  and  }\quad }
\renewcommand{\iint}[2]{\{ #1,\ldots,#2\}}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}
\newcommand{\cointLine}[1]{[#1)}
\newcommand{\ocintLine}[1]{(#1]}
\newcommand{\oointLine}[1]{(#1)}
\newcommand{\ccintLine}[1]{[#1]}


\newcommand{\boule}[2]{\operator\name{B}(#1,#2)}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\cball}[2]{\overline{\operatorname{B}}(#1,#2)}
\newcommand{\ballc}[2]{\operatorname{B}^\rmc(#1,#2)}
\newcommand{\boulefermee}[2]{\overline{\mathrm{B}}(#1,#2)}
\def\TV{\mathrm{TV}}
\newcommand\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}
\newcommand\sequenceD[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{( #1)_{ #2 \in #3} }}}

\newcommand{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}
\newcommand\sequenceDouble[4][3=,4=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ (#1_{#3},#2_{#3}) \}}}{\ensuremath{\{  (#1_{#3},#2_{#3}), \eqsp #3 \in #4 \}}}}
\newcommand{\sequencenDouble}[3][3=n\in\N]{\ensuremath{\{ (#1_{n},#2_{n}), \eqsp #3 \}}}


\newcommand{\wrt}{w.r.t.}
\newcommand{\Withoutlog}{w.l.o.g.}
\def\iid{i.i.d.}
\def\eg{e.g.}
\def\Id{\mathrm{Id}}
\def\Idd{\mathrm{I}_d}
\newcommand{\ensemble}[2]{\left\{#1\,:\eqsp #2\right\}}
\newcommand{\ensembleLigne}[2]{\{#1\,:\eqsp #2\}}
\def\rmD{\mathrm{D}}%
\def\mrd{\mathrm{D}}


\def\Tr{\mathrm{Tr}}
\def\generator{\calL}
\newcommand{\core}{\rmc}
\def\lambdac{\lambda_{\mathrm{c}}}
\def\bfe{\mathbf{e}}

  \newcommand{\pablo}[1]{\todo[color=black!20]{{\textbf PJ:} #1}}
   \newcommand{\pabloi}[1]{\todo[color=black!20,inline]{{\textbf PJ:} #1}}
 \def\a{a}
\def\domain{\mathrm{D}}
\def\card{\operatorname{card}}
\def\path{\operatorname{path}}
\def\bigone{\operatorname{1}}
\def\bigO{\mathcal{O}}
\def\Cp{C_{\operatorname{P}}}
\def\core{\mathsf{C}}
\def\entropyA{\mathscr{H}}
\def\range{\operatorname{Ran}}
\def\kernel{\operatorname{Ker}}
\def\spec{\operatorname{Spec}}

\def\ff{f}

\newcommand\overlineb[1]{{#1}}
\def\poly{\mathrm{poly}}
\def\veps{\varepsilon}
\def\trace{\operatorname{Tr}}
\def\sign{\operatorname{sgn}}
\def\diag{\operatorname{diag}}
\def\diam{\operatorname{diam}}
\newcommand\tcb[1]{\textcolor{cyan}{#1}}
\newcommand\tcbb[1]{\textcolor{blue}{#1}}
\newcommand\tcr[1]{\textcolor{red}{#1}}
\def\rateConv{\alpha}
\def\vareps{\varepsilon}
\def\sphere{\mathbb{S}}
\newcommand{\1}{\mathbbm{1}}


\newcommand{\vphi}{\varphi}
\newcommand{\vphibf}{\boldsymbol{\varphi}}
\newcommand{\even}{\mathrm{e}}

\def\restriction#1#2{\mathchoice
              {\setbox1\hbox{${\displaystyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\textstyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptscriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}}
\def\restrictionaux#1#2{{#1\,\smash{\vrule height .8\ht1 depth .85\dp1}}_{\,#2}}



\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\BWUVP}{BW_2^2-UVP}
\DeclareMathOperator{\BW}{BW_2^2}



\def\rmX{\mathrm{X}}
\def\rmVar{\mathrm{Var}}

\def\Ret{\mathrm{Ret}}

\def\bphi{\bar{\phi}}
\def\bgamma{\bar{\gamma}}

\def\loiGauss{\mathrm{N}}
\def\gauss{\loiGauss}
\def\tx{\tilde{x}}
\def\tz{\tilde{z}}



\newcommand\norme[1]{\left\Vert #1 \right\Vert}


\def\parallelTransport{\mathrm{T}}
\def\distM{\mathrm{d}_{\msm}} %
\def\distT{\rho_{\Theta}}
\def\metricM{\mathfrak{g}}
\def\vol{\mathrm{vol}}
\def\volM{\mathrm{vol}_{\msm}}
\def\grad{\mathrm{grad}\,}
\def\Hess{\mathrm{Hess}\,}
\def\teta{\tilde{\eta}}
\def\rmD{\mathrm{D}}

\def\noise{e}
\def\hnoise{\hat{e}}
\def\Exp{\mathrm{Exp}}
\def\Log{\mathrm{Log}}
\def\planT{\rmT}
\def\Cut{\mathrm{Cut}}
\def\ID{\mathrm{ID}}
\def\dupgamma{\dot{\upgamma}}


\def\grassmann{\mathrm{Gr}}
\def\stiefel{\mathrm{St}}
\def\transpose{\top}
\def\scrl{\mathscr{L}}
\def\scrlinf{\scrl_{\infty}}
\def\scrlU{\scrl^{(1)}}
\def\scrlD{\scrl^{(2)}}

\def\metric{\metricM}

\def\cu{\overline{c}}
\def\cl{\underline{c}}

\def\sigmaZ{\sigma_0^2}
\def\sigmaU{\sigma_1^2}
\def\bfb{\mathbf{b}}
\def\ttheta{\tilde{\theta}}
\def\Gammabf{\boldsymbol{\Gamma}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\def\proj{\operatorname{proj}}
\def\Leb{\mathrm{Leb}}
\def\Vdist{V_2}
\def\VHuber{V_1}
\def\thetas{{\theta^{\star}}}

\def\htheta{\hat{\theta}}
\def\hthetas{{\hat{\theta}^{\star}}}
\def\thetaspi{{\theta^{\star}_{\pi}}}
\def\supp{\mathrm{supp}}
\def\constanteC{C}

\def\ConstH{C_H}
\def\rmcl{\mathrm{Cl}}
\def\vt{\mathpzc{V}}

\renewcommand\hmmax{0}
\renewcommand\bmmax{0}
\def\bnu{\bar{\nu}}
\def\bupeta{\bar{\upeta}}
\def\tb{\tilde{b}}
\def\cupeta{\check{\upeta}}
\def\gVar{g} %
\def\gPlan{\mathrm{g}} %
\def\gInter{\mathpzc{g}} %

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\def\btheta{\bar{\theta}}
\def\tsigma{\tilde{\sigma}}
\def\tf{\tilde{f}}
\def\MKer{Q_{\upeta}}
\def\bu{\bar{u}}

\def\planTsT{\planT_{\thetas}\Theta}
\def\bouletan{\bar{\mathbb{B}}}
\def\SPD{\mathrm{Sym}}
\def\Pmeasurell{\mathscr{P}^{(\ell)}}
\def\Pmeasurem{\mathscr{P}^{(m)}}
\newcommand{\isEquivTo}[1]{\underset{#1}{\sim}}
\def\varphibf{\boldsymbol{\varphi}}
\def\densityGaussian{\gauss}

\def\SLIPS{\texttt{SLIPS}}
\def\ISLE{\texttt{ISLE}}

\def\tY{\tilde{Y}}
\def\tU{\tilde{U}}
\def\bY{\mathbf{Y}}

\newcommand{\fracD}[2]{#1/#2}




\def\bu{\bar{u}}
\def\bY{\bar{Y}}

\def\rmq{\mathrm{q}}

\def\setFunConT{\mathbf{C}_T}

\def\gammaref{\gamma^{\mathrm{ref}}}






==> header.tex <==



\usepackage{comment}
\usepackage{caption}
\usepackage[tbtags]{amsmath}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{amssymb,mathrsfs}
\usepackage{amsfonts}
\usepackage{upgreek}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{booktabs}       %
\usepackage{todonotes}
\usepackage{multirow}
\usepackage{color}
\usepackage{algpseudocode}
\usepackage[linesnumberedhidden,ruled,vlined, algo2e]{algorithm2e}
\usepackage{algorithm}
\usepackage{soul}





\usepackage{stmaryrd}

\usepackage{array}
\newcolumntype{?}{!{\vrule width 1.5pt}}

\usepackage{esvect}
\usepackage[inline]{enumitem}
\def\UrlBreaks{\do\/\do-}
\usepackage{graphicx} %
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{xcolor}
\usepackage{colortbl}
\colorlet{linkcolor}{blue!70!black}
\definecolor{pearDark}{HTML}{2980B9}
\usepackage{bbm}

\usepackage{ifthen}
\usepackage{xargs}


\usepackage{wrapfig}


\usepackage{aliascnt}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{autonum}
\makeatletter
\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}


\newtheorem*{lemma_nonumber*}{Lemma}


\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}



\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}

\newaliascnt{remark}{theorem}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}



\crefname{figure}{figure}{figures}
\Crefname{Figure}{Figure}{Figures}


\newtheorem{assumption}{\textbf{A}\hspace{-3pt}} \setcounter{assumption}{-1}
\Crefname{assumption}{\textbf{A}\hspace{-3pt}}{\textbf{A}\hspace{-3pt}}
\crefname{assumption}{\textbf{A}}{\textbf{A}}
\crefformat{assumption}{{\textbf{A}}#2#1#3}
\crefname{assumption}{assumption}{assumptions}
\Crefname{Assumption}{Assumption}{Assumptions}

\newtheorem{assumptionF}{\textbf{F}\hspace{-3pt}}
\crefformat{assumptionF}{{\textbf{F}}#2#1#3}

\newenvironment{assumptionbis}[1]
  {\renewcommand{\theassumptionF}{\ref*{#1}$\mathbf{b}$}%
   \addtocounter{assumptionF}{-1}%
   \begin{assumptionF}}
  {\end{assumptionF}}



\newtheorem{assumptionB}{\textbf{B}\hspace{-3pt}}
\Crefname{assumptionB}{\textbf{B}\hspace{-3pt}}{\textbf{B}\hspace{-3pt}}
\crefname{assumptionB}{\textbf{B}}{\textbf{B}}

\newtheorem{assumptionC}{\textbf{C}\hspace{-3pt}}
\Crefname{assumptionC}{\textbf{C}\hspace{-3pt}}{\textbf{C}\hspace{-3pt}}
\crefname{assumptionC}{\textbf{C}}{\textbf{C}}


\newtheorem{assumptionH}{\textbf{H}\hspace{-3pt}}
\Crefname{assumptionH}{\textbf{H}\hspace{-3pt}}{\textbf{H}\hspace{-3pt}}
\crefname{assumptionH}{\textbf{H}}{\textbf{H}}

\newtheorem{assumptionT}{\textbf{T}\hspace{-3pt}}
\Crefname{assumptionT}{\textbf{T}\hspace{-3pt}}{\textbf{T}\hspace{-3pt}}
\crefname{assumptionT}{\textbf{T}}{\textbf{T}}

\newtheorem{assumptionD}{\textbf{D}\hspace{-3pt}}
\Crefname{assumptionT}{\textbf{T}\hspace{-3pt}}{\textbf{T}\hspace{-3pt}}
\crefname{assumptionT}{\textbf{T}}{\textbf{T}}


\newtheorem{assumptionL}{\textbf{L}\hspace{-3pt}}
\Crefname{assumptionL}{\textbf{L}\hspace{-3pt}}{\textbf{L}\hspace{-3pt}}
\crefname{assumptionL}{\textbf{L}}{\textbf{L}}

\newtheorem{assumptionQ}{\textbf{Q}\hspace{-3pt}}
\Crefname{assumptionQ}{\textbf{Q}\hspace{-3pt}}{\textbf{Q}\hspace{-3pt}}
\crefname{assumptionQ}{\textbf{Q}}{\textbf{Q}}


\newtheorem{assumptionAR}{\textbf{AR}\hspace{-3pt}}
\Crefname{assumptionAR}{\textbf{AR}\hspace{-3pt}}{\textbf{AR}\hspace{-3pt}}
\crefname{assumptionAR}{\textbf{AR}}{\textbf{AR}}

\makeatletter
\newcommand*{\centerfloat}{%
  \parindent \z@
  \leftskip \z@ \@plus 1fil \@minus \textwidth
  \rightskip\leftskip
  \parfillskip \z@skip}
\makeatother

\usetikzlibrary{spy}
\usetikzlibrary[patterns] %
\usetikzlibrary{calc,decorations.pathreplacing} %
\usetikzlibrary{shadows.blur} %
\usetikzlibrary{shapes.symbols}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

